On Simultaneous Two-player Combinatorial Auctions

We consider the following communication problem: Alice and Bob each have some valuation functions $v_1(\cdot)$ and $v_2(\cdot)$ over subsets of $m$ items, and their goal is to partition the items into $S, \bar{S}$ in a way that maximizes the welfare, $v_1(S) + v_2(\bar{S})$. We study both the allocation problem, which asks for a welfare-maximizing partition and the decision problem, which asks whether or not there exists a partition guaranteeing certain welfare, for binary XOS valuations. For interactive protocols with $poly(m)$ communication, a tight 3/4-approximation is known for both [Fei06,DS06]. For interactive protocols, the allocation problem is provably harder than the decision problem: any solution to the allocation problem implies a solution to the decision problem with one additional round and $\log m$ additional bits of communication via a trivial reduction. Surprisingly, the allocation problem is provably easier for simultaneous protocols. Specifically, we show: 1) There exists a simultaneous, randomized protocol with polynomial communication that selects a partition whose expected welfare is at least $3/4$ of the optimum. This matches the guarantee of the best interactive, randomized protocol with polynomial communication. 2) For all $\varepsilon > 0$, any simultaneous, randomized protocol that decides whether the welfare of the optimal partition is $\geq 1$ or $\leq 3/4 - 1/108+\varepsilon$ correctly with probability $> 1/2 + 1/ poly(m)$ requires exponential communication. This provides a separation between the attainable approximation guarantees via interactive ($3/4$) versus simultaneous ($\leq 3/4-1/108$) protocols with polynomial communication. In other words, this trivial reduction from decision to allocation problems provably requires the extra round of communication.

==> bxos.tex <==
%!TEX root = MAIN.tex

\subsection{Simultaneous protocol for two BXOS parties (implies Theorem~\ref{thm:mainupper})}
\label{sec:bxos}
\begin{algorithm}
	\floatname{algorithm}{Protocol}
        \caption{Simultaneous protocol for 2-party combinatorial auctions with binary XOS valuations}
        \label{pro:bi2}
    \begin{algorithmic}[1]
	\STATE Alice computes the $(k,1/2)$-sketch $(b_1,...,b_k)$ of her valuation $v_1$. Then she picks $j$ uniformly randomly from $\{1,...,k\}$ and sends $b_j$ to the auctioneer.
	\STATE For each item $i$, the auctioneer allocates it to Alice if $b_j(\{i\}) =1$; otherwise allocate it to Bob. 
             \end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:simbxos}
Protocol \ref{pro:bi2} gives a $(3/4-1/k)$-approximation in expectation to the 2-party BXOS allocation problem. 
\end{theorem}

Recall that this is tight, as even randomized, interactive protocols require exponential communication to beat a $3/4$-approximation.

\subsection{Sequential protocol for multiple BXOS parties}
\label{sec:bxosm}
\begin{algorithm}[ht]
	\floatname{algorithm}{Protocol}
        \caption{Sequential protocol for multi-party combinatorial auctions with binary XOS valuations}
       \label{pro:bin}
    \begin{algorithmic}[1]
    	\FOR {$l = 1,...,n-1$}
	\STATE The $l$-th player computes the $(k,1/2)$-sketch $(b^l_1,...,b^l_k)$ of her valuation $v_l$ for items that are left. Then she picks $j$ uniformly randomly from $\{1,...,k\}$ and broadcasts $b^l_j$.
	\STATE For each item $i$ left, the auctioneer allocates it to the $l$-th player if $b^l_j(\{i\}) =1$.
       	\ENDFOR
	\STATE Allocate the left items to the $n$-th player.
       \end{algorithmic}

\end{algorithm}
\begin{theorem}
\label{thm:simbxosm}
Protocol \ref{pro:bin} gives a $(1/2-1/k)$-approximation in expectation to the $n$-party BXOS allocation problem. 
\end{theorem}

Note that this is not tight - \cite{DobzinskiS06,Feige06} provide a poly-communication $1-1/e$ approximation, but Protocol~\ref{pro:bin} is considerably simpler.

==> simulintro.tex <==
%!TEX root = MAIN.tex

\cite{Yao:1979:CQR:800135.804414} proposed the 2-party simultaneous communication model when communication complexity was introduced. \cite{Papadimitriou:1982:CC:800070.802192}, \cite{Duris:1984:LBC:800057.808668}, \cite{Nisan:1993:RCC:152322.152386} showed that in the 2-party case, there is an exponential gap between $k$ and $(k-1)$-round deterministic/randomized communication complexity of an explicit function. In the multiparty number-on-forehead communication model \cite{ChandraFL83b}, \cite{BabaiGKL03} showed an exponential gap between simultaneous communication complexity and communication complexity for up to $(\log n)^{1-\varepsilon}$ players for any $\varepsilon >0$. \cite{DobzinskiNO14} recently showed that in combinatorial auctions with unit demand bidders/subadditive bidders, there is an exponential gap (exponential in the number of players) between simultaneous communication complexity and communication complexity.

==> truthful.tex <==
%!TEX root = MAIN.tex

\subsection{Truthful mechanism for multiple binary XOS parties}
\label{sec:mechanisms}
In this section, we will show how to transform Protocol \ref{pro:bi2} and Protocol \ref{pro:bin} into truthful mechanisms. Since Protocol \ref{pro:bi2} is a special case of Protocol \ref{pro:bin}, we will only do the transformation for Protocol \ref{pro:bin}. 

\begin{algorithm}[ht]
	\floatname{algorithm}{Mechanism}
        \caption{Truthful mechanism for multi-party combinatorial auctions with binary XOS valuations}
       \label{mech:bin}
    \begin{algorithmic}[1]
    	\FOR {$l = 1,...,n-1$}
	\STATE The $l$-th player broadcasts $k$ binary additive valuations $(b^l_1,...,b^l_k)$. 
	\STATE The auctioneer picks $j$ uniformly randomly from $\{1,...,k\}$ and broadcasts $j$. For each item $i$ left, the auctioneer allocates it to the $l$-th player if $b^l_j(\{i\}) =1$ and charges the $l$-th player $\frac{\sum_{j' =1}^k b^l_{j'}(\{i\})}{2k}$.
       	\ENDFOR
	\STATE Allocate the left items to the $n$-th player.
       \end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:truthful}
In Mechanism \ref{mech:bin}, for any $l \in \{1,...,n-1\}$ and any history before the $l$-player, if $(b^l_1,...,b^l_k)$ maximizes her expected utility, then $(b^l_1,...,b^l_k)$ is a $(k, 1/2)$-sketch of $v_l$ for items left.
\end{theorem}

Note that this is not tight - a simple observation shows how to turn the $(1-1/e)$-approximation of~\cite{Feige06, DobzinskiS06} into a truthful mechanism for binary XOS bidders. One noteworthy difference is that in Mechanism~\ref{mech:bin}, following the intended protocol is \emph{strictly} more profitable than any deviation. In the previous mechanisms, all bidders get zero utility no matter what they do. Mechanism~\ref{mech:bin} is also considerably simpler than the previous mechanisms.

==> xos.tex <==
%!TEX root = MAIN.tex

\subsection{Simultaneous protocol for two XOS parties (implies part of Theorem~\ref{thm:mainlower})}\label{sec:xos}
\begin{algorithm}[ht]
	\floatname{algorithm}{Protocol}
        \caption{Deterministic, simultaneous protocol for 2-party combinatorial auctions with  XOS valuations}
        \label{pro:xos2}
    \begin{algorithmic}[1]
	\STATE Alice sends the $(k,1/3)$-sketch $(b^1_1,...,b^1_k)$ of her valuation $v_1$ and Bob sends the  $(k,1/3)$-sketch $(b^2_1,...,b^2_k)$ of his valuation $v_2$ simultaneously to the auctioneer.
	\STATE \textbf{For allocation problem:} Auctioneer finds $j,j'$ maximize $\SW(b^1_j, b^2_{j'})$ and allocates items using the allocation that achieves $\SW(b^1_j, b^2_{j'})$. 
	\STATE \textbf{For decision problem:} Let $X$ be the parameter in the decision problem. Auctioneer finds $j,j'$ maximize $\SW(b^1_j, b^2_{j'})$. If $\SW(b^1_j, b^2_{j'}) \geq (23/32-1/k)X$, say "yes" ($\SW(v_1,v_2) \geq X$). If $\SW(b^1_j, b^2_{j'}) < (23/32-1/k)X$,  say "no". 
             \end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:simxos}
Protocol \ref{pro:xos2} gives a $(23/32 -1/k)$-approximation to the 2-party XOS allocation problem and the 2-party XOS decision problem. 
\end{theorem}

While we don't know whether or not $23/32$ is in general tight for simultaneous protocols for XOS valuations, the analysis of Protocol~\ref{pro:xos2} (and protocols like it) is indeed tight:
\begin{lemma}
\label{lem:xoslb}
For any constant $\varepsilon > 0$, there exist binary XOS valuations $v_1$ and $v_2$ with sufficiently large $m$ such that simultaneous protocols in the following form won't get $\SW(b^1_j, b^2_{j'})$ larger than $(23/32 + 2\varepsilon)\SW(v_1,v_2)$:
\begin{enumerate}
\item Alice sends the $(k_1,\alpha_1)$-sketch $(b^1_1,...,b^1_{k_1})$ of her valuation $v_1$ and Bob sends the  $(k_2,\alpha_2)$-sketch $(b^2_1,...,b^2_{k_2})$ of his valuation $v_2$ simultaneously to the auctioneer. ($0\leq \alpha_1,\alpha_2 \leq 1/2$, $k_1,k_2$ can be any positive integer)
\item Auctioneer finds $j,j'$ maximize $\SW(b^1_j, b^2_{j'})$ and allocates items using the allocation that achieves $\SW(b^1_j, b^2_{j'})$. 
\end{enumerate}
\end{lemma}


\subsection{Two-round protocol for two XOS parties} \label{sec:xos2r}

\begin{algorithm}
	\floatname{algorithm}{Protocol}
        \caption{Two-round, deterministic protocol for 2-party combinatorial auctions with XOS valuations}
        \label{pro:2rxos2}
    \begin{algorithmic}[1]
	\STATE Alice computes the $(k,1/2)$-sketch $(b_1,...,b_k)$ of her valuation $v_1$ and sends it to Bob. Bob find $j$ that maximize $SW(b_j, v_2)$, and sends $SW(b_j,v_2)$ together with the allocation that achieves $SW(b_j,v_2)$ to the auctioneer.
	\STATE \textbf{For allocation problem:} The auctioneer allocates items according to the allocation provided by Bob.
	\STATE \textbf{For decision problem:} Let $X$ be the parameter in the decision problem. If $SW(b_j, v_2) \geq (3/4-1/k)X$, say "yes" ($\SW(v_1,v_2) \geq X$). If $SW(b_j, v_2) < (3/4-1/k)X$, say "no". 
             \end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:2rxos2}
Protocol \ref{pro:2rxos2} gives a $(3/4-1/k)$-approximation to the 2-party XOS allocation problem and the 2-party XOS decision problem. 
\end{theorem}

Note that this is tight, as exponential communication is required to beat a $3/4$-approximation in any number of rounds. A $3/4$-approximation in more rounds is indeed already known~\cite{DobzinskiS06, Feige06}, but the above protocol is considerably simpler.


